Python Tool for Visualizing Variability of Pareto Fronts over Multiple Runs

Hyperparameter optimization is crucial to achieving high performance in deep learning. On top of the performance, other criteria such as inference time or memory requirement often need to be optimized due to some practical reasons. This motivates research on multi-objective optimization (MOO). However, Pareto fronts of MOO methods are often shown without considering the variability caused by random seeds and this makes the performance stability evaluation difficult. Although there is a concept named \emph{empirical attainment surface} to enable the visualization with uncertainty over multiple runs, there is no major Python package for empirical attainment surface. We, therefore, develop a Python package for this purpose and describe the usage. The package is available at https://github.com/nabenabe0928/empirical-attainment-func. OptunaHub now provides our implementation at https://hub.optuna.org/visualization/plot_empirical_attainment_surface/.

==> settings/labels-in-main.tex <==
\ifappendix
% Do nothing

\else

% Define the labels in the main sections
\customlabel{data1}{1}
\customlabel{data2}{2}

% Start numberings of each data as if
% appendix takes over the numbering from the main section
\renewcommand\thefigure{\arabic{figure}}
\setcounter{figure}{1}  % start from 2
\renewcommand\thetable{\arabic{table}}
\setcounter{table}{2}  % start from 3
\renewcommand\thealgorithm{\arabic{algorithm}}
\setcounter{algorithm}{3}  % start from 4
\renewcommand\theequation{\arabic{equation}}
\setcounter{equation}{4}  % start from 5

% Change the numbering of sections to Alphabetic
\renewcommand{\thesection}{\Alph{section}} 
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesection.\arabic{subsection}.\arabic{subsubsection}}

\fi

